Limited Communications Distributed Optimization via Deep Unfolded Distributed ADMM

Distributed optimization is a fundamental framework for collaborative inference and decision making in decentralized multi-agent systems. The operation is modeled as the joint minimization of a shared objective which typically depends on observations gathered locally by each agent. Distributed optimization algorithms, such as the common D-ADMM, tackle this task by iteratively combining local computations and message exchanges. One of the main challenges associated with distributed optimization, and particularly with D-ADMM, is that it requires a large number of communications, i.e., messages exchanged between the agents, to reach consensus. This can make D-ADMM costly in power, latency, and channel resources. In this work we propose unfolded D-ADMM, which follows the emerging deep unfolding methodology to enable D-ADMM to operate reliably with a predefined and small number of messages exchanged by each agent. Unfolded D-ADMM fully preserves the operation of D-ADMM, while leveraging data to tune the hyperparameters of each iteration of the algorithm. These hyperparameters can either be agent-specific, aiming at achieving the best performance within a fixed number of iterations over a given network, or shared among the agents, allowing to learn to distributedly optimize over different networks. For both settings, our unfolded D-ADMM operates with limited communications, while preserving the interpretability and flexibility of the original D-ADMM algorithm. We specialize unfolded D-ADMM for two representative settings: a distributed estimation task, considering a sparse recovery setup, and a distributed learning scenario, where multiple agents collaborate in learning a machine learning model. Our numerical results demonstrate that the proposed approach dramatically reduces the number of communications utilized by D-ADMM, without compromising on its performance.

==> abstract_heb.tex <==
\thispagestyle{empty}
\selectlanguage{hebrew}

\begin{center}
    \Large
     \textbf{אופטימיזציה מבוזרת לתקשורת מוגבלת בשיטת כיוון לסירוגין של מכפילים דרך פרישה עמוקה} 

    \vspace{0.4cm}
    \large
    יואב נח
       
    \vspace{0.4cm}
    \large
    עבודת גמר לתואר מוסמך למדעי הטבע
      
    \vspace{0.2cm}
    \large
    אוניברסיטת בן-גוריון בנגב
    
    \vspace{0.2cm}
    \large
    
    \selectlanguage{english}
    2023
    
    \selectlanguage{hebrew}
    \vspace{0.9cm}
    \Large
    \textbf{תקציר}
\end{center}
אופטימיזציה מבוזרת היא מסגרת בסיסית להסקת שיתוף פעולה וקבלת החלטות במערכות מרובות סוכנים מרכזיות. הפעולה מעוצבת כמזעור משותף של מטרה משותפת שבדרך כלל תלוי בתצפיות שנאספו באופן מקומי על ידי כל סוכן. אלגוריתמי אופטימיזציה משותפים, כגון המשותף המבוזר שיטת כיוון לסירוגין של מכפילים, להתמודד משימה זו על ידי שילוב איטרטיבי של חישובים ומסר מקומיים
חילופים. אחד האתגרים העיקריים הקשורים לאופטימיזציה מבוזרת, ובמיוחד עם כיוון לסירוגין של מכפילים היא שהיא דורשת
מספר רב של תקשורת, כלומר, הודעות שהוחלפו בין הסוכנים בשביל להגיע לקונצנזוס. זה יכול להפוך את שיטת כיוון לסירוגין של מכפילים ליקר בהספק, בהשהייה ובמשאבי ערוץ. בעבודה זו אנחנו מציעים כיוון לסירוגין של מכפילים פרוש, העוקב אחר העומק המתהווה. פיתוח מתודולוגיה זו מאפשרת לכיוון לסירוגין של מכפילים לפעול בצורה אמינה עם מספר מוגדר מראש וקטן של הודעות שהוחלפו על ידי כל סוכן. כיוון לסירוגין של מכפילים פרוש שומר באופן מלא על פעולתו של כיוון לסירוגין של מכפילים, תוך מינוף נתונים לכוונון ההיפרפרמטרים של כל איטרציה של האלגוריתם. ההיפרפרמטרים האלה יכולים גם כן
להיות ספציפי לסוכן, במטרה להשיג את הביצועים הטובים ביותר בתוך מספר קבוע של איטרציות ברשת נתונה, או משותפות בין הסוכנים, מה שמאפשר ללמוד לבצע אופטימיזציה מבוזרת
רשתות שונות. עבור שתי ההגדרות, הכיוון לסירוגין של מכפילים הפרוש שלנו פועל עם תקשורת מוגבלת, תוך שמירה על
פרשנות וגמישות של אלגוריתם כיוון לסירוגין של מכפילים המקורי.
אנו מתמחים בכיוון לסירוגין של מכפילים פרוש עבור שתי הגדרות מייצגות: משימת הערכה מבוזרת, בהתחשב בהתאוששות דלילה הגדרה, ותרחיש למידה מבוזרת, שבו מספר סוכנים לשתף פעולה בלימוד מודל למידת מכונה. המספרי שלנו התוצאות מראות שהגישה המוצעת באופן דרמטי מפחית את מספר התקשורת בשימוש על ידי  כיוון לסירוגין של מכפילים מבלי להתפשר על הביצועים שלו.


\selectlanguage{english}

==> cover_heb.tex <==

\begin{titlepage}
    \begin{center}
        \vspace*{1cm}
        
        \includegraphics[width=0.1\textwidth]{figs/bgu.png}\\
        \selectlanguage{hebrew}אוניברסיטת בן-גוריון בנגב\\הפקולטה למדעי הטבע\\המחלקה למדעי המחשב\selectlanguage{english}

        \vspace{2cm}
        
        \selectlanguage{hebrew}
        {\Large \textbf{אופטימיזציה מבוזרת לתקשורת מוגבלת בשיטת כיוון לסירוגין של מכפילים דרך פרישה עמוקה}}
        \selectlanguage{english}
        
        \vspace{1.5cm}

        \selectlanguage{hebrew}
        חיבור זה מהווה חלק מהדרישות לקבלת התואר מוסמך למדעי הטבע\selectlanguage{english}(M.Sc)
        \vspace{1cm}
        
        \selectlanguage{hebrew}
        יואב נח
        \selectlanguage{english}
        \vspace{1cm}

        \selectlanguage{hebrew}
        בהנחיית ד"ר ניר שלזינגר 
        \selectlanguage{english}
        
        \vfill
        \selectlanguage{hebrew}
        ספטמבר \quad
        \selectlanguage{english}
        2023
     \end{center}
\end{titlepage}

==> cover_page.tex <==
\begin{titlepage}
    \begin{center}
        \vspace*{1cm}
        
        \includegraphics[width=0.1\textwidth]{Main_pages/bgu.png}\\
        Ben-Gurion University of the Negev\\
        The Faculty of Natural Sciences\\
        The Department of Computer Science
        
        \vspace{2cm}
        
        {\Large \thesistitle}
        
        \vspace{1cm}
        
        Thesis submitted in partial fulfillment of the requirements\\for the Master of Sciences degree
        
        \vspace{1cm}
        
        \thesisauthorname
        
        \vspace{1cm}
        
        Under the supervision of \thesissupervisername
        
        \vfill
        
        \thesismonth \quad \thesisyear

    \end{center}
\end{titlepage}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
